Meta-Meta Classification for One-Shot Learning

We present a new approach, called meta-meta classification, to learning in small-data settings. In this approach, one uses a large set of learning problems to design an ensemble of learners, where each learner has high bias and low variance and is skilled at solving a specific type of learning problem. The meta-meta classifier learns how to examine a given learning problem and combine the various learners to solve the problem. The meta-meta learning approach is especially suited to solving few-shot learning tasks, as it is easier to learn to classify a new learning problem with little data than it is to apply a learning algorithm to a small data set. We evaluate the approach on a one-shot, one-class-versus-all classification task and show that it is able to outperform traditional meta-learning as well as ensembling approaches.

==> sec_algo.tex <==
\begin{figure}
  \centering
    \begin{align*}
    & S ::= op(T_0, T_1, … T_m) \mid A \\
    & T ::= op(A_0, A_1, ...A_n) \mid A \\
    & A ::= f_0 \mid f_1 \mid \ldots \mid f_r \\
    \end{align*}
\caption{Grammar for generating 2-level sparse architectures. $f_i$ are the input features $op$ is a perceptron operator.}
\label{fig:grammar}
\end{figure}


Our method relies on a meta-learning based approach where the learning happens in two phases. In the first phase which is offline, we generate a corpus of data and learn a meta-model that can efficiently search a sparse classifier architecture suitable for a single given image of an object. In the second phase which is online, we train the classifier for a few epochs on that single image and a number of images of other objects. First we will describe the offline meta-model learning process, then describe the online learning.

\subsection{Meta-model}

In order to search a suitable sparse classifier architecture, we design a functional programming language that generates a tree shaped architecture using the pretrained features of an image. For simplicity, we restrict the depth of the tree to two. Figure \ref{fig:grammar} shows the grammar to generate a 2-level sparse architecture. Here $f_i$ denotes the $i$th feature of an image and $op$ denotes a simple perceptron with some non-linear activation function. The meta-model is trained offline on a corpus of such architectures. We generate the corpus using a greedy heuristic in which we randomly choose an image and simulate an architecture from the root to find the top $K$ architectures at every step, where $K$ is a design choice, generally kept at a small number. In order to measure the `goodness' of an architecture given an image, we simulate the one-shot classification task, that is, train the classifier for a few epochs using the given image and $N$ randomly chosen images from other classes, and then measure the test accuracy on $N$ other images from both the target class as well as randomly chosen other classes. While generating a tree architecture, we start from the smallest possible architecture, that is, a single feature and then use two types of mutations to grow it. The first set of mutations decide which new feature will be added to the lower level of the tree and the second set of mutations decide which new feature will be added to the top level. For simplicity, the mutations allow addition of features only to the rightmost branch of the tree. They also allow any number of additions of a particular feature. While  doing the greedy simulations, we keep both the top $K$ architectures as well as the rest of the architectures in the corpus. Then our meta-model tries to learn a classifier that can separate the good architectures from the bad ones given an image.

The inputs to the meta-model are the pretrained features of a particular image, an architecture and a label whether the architecture is good or bad for the given image. We encode the architecture using a Tree LSTM. The one-hot encoding of the features present in the architecture are fed to this Tree LSTM through a fully connected (fc) layer. The image features are then concatenated with the encoded architecture through another fc layer, which finally passes through some fc layers to output a probability of whether the architecture is good or not.


